Planck 2018 results. X. Constraints on inflation

We report on the implications for cosmic inflation of the 2018 Release of the Planck CMB anisotropy measurements. The results are fully consistent with the two previous Planck cosmological releases, but have smaller uncertainties thanks to improvements in the characterization of polarization at low and high multipoles. Planck temperature, polarization, and lensing data determine the spectral index of scalar perturbations to be $n_\mathrm{s}=0.9649\pm 0.0042$ at 68% CL and show no evidence for a scale dependence of $n_\mathrm{s}.$ Spatial flatness is confirmed at a precision of 0.4% at 95% CL with the combination with BAO data. The Planck 95% CL upper limit on the tensor-to-scalar ratio, $r_{0.002}<0.10$, is further tightened by combining with the BICEP2/Keck Array BK15 data to obtain $r_{0.002}<0.056$. In the framework of single-field inflationary models with Einstein gravity, these results imply that: (a) slow-roll models with a concave potential, $V" (\phi) < 0,$ are increasingly favoured by the data; and (b) two different methods for reconstructing the inflaton potential find no evidence for dynamics beyond slow roll. Non-parametric reconstructions of the primordial power spectrum consistently confirm a pure power law. A complementary analysis also finds no evidence for theoretically motivated parameterized features in the Planck power spectrum, a result further strengthened for certain oscillatory models by a new combined analysis that includes Planck bispectrum data. The new Planck polarization data provide a stringent test of the adiabaticity of the initial conditions. The polarization data also provide improved constraints on inflationary models that predict a small statistically anisotropic quadrupolar modulation of the primordial fluctuations. However, the polarization data do not confirm physical models for a scale-dependent dipolar modulation.

==> Tables/Table_r_rev4_BK14_rounded.tex <==
\begin{table*}[!ht]
\begin{center}
\begin{tabular}{ccccc}
\noalign{\hrule\vskip 2pt}
\noalign{\hrule\vskip 3pt}
Cosmological model & Parameter & \Planck\ TT,TE,EE & \Planck\ TT,TE,EE & \Planck\ TT,TE,EE \\
$\Lambda$CDM+$r$ & & +lowEB+lensing & +lowE+lensing+BK14 & +lowE+lensing+BK14+BAO \\
\noalign{\hrule\vskip 2pt}
%Inflationary & $\ln B_{0X}$ & $\Delta \chi^2$ \\
%Model & & \\
%\hline


\multirow{2}{*}{} & $r$ & $< 0.11$ & $< 0.070$ & $< 0.070$ \\
& $r_{0.002}$ &  $<0.10$ & $< 0.064$ &$ < 0.065$ \\
& $n_{\mathrm{s}}$ & $0.9659 \pm 0.0041$ & $0.9653 \pm 0.0041$ & $0.9670 \pm 0.0037$ \\


\noalign{\hrule\vskip 2pt}
& $r$ & $< 0.16$  & $< 0.079 $ & $< 0.076$\\
& $r_{0.002}$ &  $ < 0.16$ & $< 0.077$  & $< 0.072$ \\
+$d n_{\mathrm{s}}/d \ln k$ & $n_{\mathrm{s}}$ & $ 0.9647 \pm 0.0044$
& $ 0.9640 \pm 0.0043$ & $0.9658 \pm 0.0038$ \\
& $d n_{\mathrm{s}}/d \ln k$ & $ - 0.0085 \pm 0.0073$
& $ -0.0071\pm 0.0068$ & $-0.0065 \pm 0.0066$ \\


\noalign{\hrule\vskip 2pt}
& $r$ &  $< 0.092$ & $< 0.071$ & $< 0.072$ \\
& $r_{0.002}$ &  $< 0.085$ & $< 0.065$ & $< 0.067$ \\
+$N_\mathrm{eff}$ & $n_{\mathrm{s}}$
& $0.9607_{-0.0084}^{+0.0086}$ & $ 0.9606_{-0.0083}^{+0.0084}$ & $0.9660\pm 0.0070 $\\[0.2ex]
& $N_\mathrm{eff}$  & $2.92 \pm 0.19$ & $ 2.93\pm 0.19$ & $3.02 \pm 0.17 $ \\[0.5ex]



%\noalign{\hrule\vskip 2pt}
%& $r$  & $< 0.14$ & $< 0.12$ & $<0.12$ \\
%+$Y_\mathrm{He}$
%& $n_{\mathrm{s}}$ & $0.975 \pm 0.007$ & $0.973 \pm 0.009$ & $0.969 \pm 0.008$ \\
%$r_{0.002}$ &  $< 0.142$ & < 0.117 & $< 0.112$ \\
%& $Y_\mathrm{He}$  & $0.258 \pm 0.022$ & $0.257 \pm 0.022$ & $0.252 \pm 0.014$ \\
%& $Y_\mathrm{He}$  & $0.2577^{+0.0218}_{-0.0217}$ & $0.2574^{+0.0218}_{-0.0217}$ & $0.2524^{+0.0136}_{-0.0135}$ \\



\noalign{\hrule\vskip 2pt}
& $r$  &  $< 0.097$ & $< 0.071$ & $< 0.070$ \\
& $r_{0.002}$ &  $< 0.091$ & $< 0.065$ & $< 0.065$ \\
+$m_\nu$ & $n_\mathrm{s}$ & $0.9654 \pm 0.0044$ & $ 0.9652 \pm 0.0042$ & $0.9669\pm 0.0037$\\
& $\sum m_\nu$ [eV] & $< 0.24$ & $< 0.22$ &  $< 0.11$ \\
%$r_{002}$ &  $< 0.143$ & \textcolor{red}{$< X$} & $< 0.145$ \\
%& $\Omega_K$ & $-0.008^{+0.010}_{-0.008}$  & $-0.001 \pm 0.003$ &
%$-0.045^{+0.016}_{-0.020}$ \\[0.5ex]



\noalign{\hrule\vskip 2pt}
& $r$ & $< 0.12$  & $< 0.076$ & $< 0.074$ \\
& $r_{0.002}$ &  $< 0.12$ & $<0.072$ & $< 0.068$ \\
+$\Omega_K$ & $n_{\mathrm{s}}$ & $0.9703_{-0.0046}^{+0.0045}$ & $ 0.9699_{-0.0046}^{+0.0047}$ & $0.9664_{-0.0046}^{+0.0045}$\\[0.3ex]
& $\Omega_K$ & $-0.012_{-0.006}^{+0.007}$ & $ -0.012_{-0.006}^{+0.007}$ & $0.0006\pm 0.0019 $\\[0.5ex]



\noalign{\hrule\vskip 2pt}
& $r$ &  $< 0.11$ & $< 0.074$ & $< 0.073$ \\
& $r_{0.002}$ &  $< 0.10$ & $<0.069$ & $< 0.068$ \\
+$w_0$ & $n_{\mathrm{s}}$ & $0.9675 \pm 0.0042$ & $ 0.9670 \pm 0.0042$ & $0.9660_{-0.0040}^{+0.0039}$\\[0.3ex]
%& $w$ & $-1.581_{-0.334}^{+0.150}$ & $ -1.584_{-0.336}^{+0.153}$ & $-1.044_{-0.050}^{+0.057} $\\[0.5ex]
& $w_0$ & $-1.58_{-0.34}^{+0.14}$ & $ -1.58_{-0.34}^{+0.14}$ & $-1.04_{-0.05}^{+0.06} $\\[0.5ex]
\hline
\end{tabular}
\end{center}
\caption{Constraints on the tensor-to-scalar ratio $r$ and scalar tilt $n_\mathrm{s}$ 
for the $\Lambda$CDM+$r$ model and some important extensions and different data sets. 
For each model we quote 68\,\% confidence limits on measured parameters and 
95\,\% upper bounds on other parameters.}
\label{tab:r_extended}
\end{table*}



==> Tables/table_inflationarymodels_bk14.tex <==
%\newcommand{\pz}{\phantom{0}}
%\newcommand{\pzz}{\phantom{00}}
%\newcommand{\pd}{\phantom{-}}

%\begin{landscape}
\begin{table*}
\begin{center}
%\footnotesize
%\scriptsize
%\begin{tabular}{lrrrrrrrr}
\begin{tabular}{lccrr}
\noalign{\hrule\vskip 2pt} \noalign{\hrule\vskip 3pt}
%\hline
%\vspace{.3cm}
%Inflationary & Potential & Prior(s) & $\Delta n$ & $\Delta\chi^2$& $\ln B$ \\
%Model & & & & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) \\  
%Inflationary Model & Potential $V(\phi)$ & Prior(s) & $\Delta\chi^2_{R^2}$ & $\Delta \ln \mathcal{E}_{R^2}$ \\
%Inflationary Model & Potential $V(\phi)$ & Parameter range & $\Delta\chi^2_{R^2}$ & $\Delta \ln \mathcal{E}_{R^2}$ \\
Inflationary model & Potential $V(\phi)$ & Parameter range & $\Delta\chi^2$ & $\ln B$ \\
%& & & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) \\
%& & & & \\
\noalign{\hrule\vskip 3pt}
%General models:
%& & & & \\
$R + R^2/(6 M^2)$ & $\Lambda^4 \left( 1 - e^{- \sqrt{2/3} \phi/M_\mathrm{Pl} } \right)^2$ & \dots & \dots & $ \dots $ \\
\noalign{\vskip 2pt}
%& & & & \\
%\citep{Starobinsky:1980te,Mukhanov:1981xt,Starobinsky:1983zz}& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $0 \le p \le 4$ & \dots & \dots & $-$ \\
%\citep{Linde:1983gd} & & & & \\
%& & & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 2/3$ & $2.8$ & $-2.6$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^{2/3}$ & \dots & $2.8$ & $-2.6$ \\
Power-law potential & $\lambda M_\mathrm{Pl}^{10/3} \phi^{2/3}$ & \dots & $2.8$ & $-2.6$ \\
\noalign{\vskip 2pt}
%& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 1$ & $2.5$ & $-1.9$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)$ & \dots & $2.5$ & $-1.9$ \\
Power-law potential & $\lambda M_\mathrm{Pl}^3 \phi$ & \dots & $2.5$ & $-1.9$ \\
\noalign{\vskip 2pt}
%& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 4/3$ & $10.4$ & $-4.5$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^{4/3}$ & \dots & $10.4$ & $-4.5$ \\
Power-law potential & $\lambda M_\mathrm{Pl}^{8/3} \phi^{4/3}$ & \dots & $10.4$ & $-4.5$ \\
\noalign{\vskip 2pt}
%& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 2$ & $22.3$ & $-7.1$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^2$ & \dots & $22.3$ & $-7.1$ \\
Power-law potential & $\lambda M_\mathrm{Pl}^2 \phi^2$ & \dots & $22.3$ & $-7.1$ \\
\noalign{\vskip 2pt}
%& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 3$ & $40.9$ & $-19.2$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^3$ & \dots & $40.9$ & $-19.2$ \\
Power-law potential & $\lambda M_\mathrm{Pl} \phi^3$ & \dots & $40.9$ & $-19.2$ \\
\noalign{\vskip 2pt}
%& & & & \\
%Power-law potentials & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^p$ & $p = 4$ & $-$ & $-33.3$ \\
%Power-law potential & $\Lambda^4 \left( \phi / M_\mathrm{Pl} \right)^4$ & \dots & $-$ & $-33.3$ \\
Power-law potential & $\lambda \phi^4$ & \dots & $89.1$ & $-33.3$ \\
\noalign{\vskip 2pt}
%& & & & \\
Non-minimal coupling & $\lambda^4 \phi^4 + \xi \phi^2 R/2 $ & $-4 < \log_{10} \xi < 4$ & $3.1$ & $-1.6$ \\
\noalign{\vskip 2pt}
%& & & & \\
%\hline
Natural inflation & $\Lambda^4 \left[ 1+\cos \left( \phi / f \right) \right]$ & $0.3 < \log_{10} (f/M_\mathrm{Pl}) < 2.5$ & $9.4$ & $-4.2$ \\
\noalign{\vskip 2pt}
%& & & & \\
Hilltop quadratic model & $\Lambda^4 \left( 1 - \phi^2 / \mu_2^2 + \dots \right)$ & $0.3 < \log_{10} (\mu_2 /M_\mathrm{Pl}) < 4.85$ & $1.7$ & $-2.0$ \\
\noalign{\vskip 2pt}
%\citep{Boubekeur:2005zm}
%& & & & \\
Hilltop quartic model & $\Lambda^4 \left( 1 - \phi^4 / \mu_4^4 + \dots \right)$ & $-2 < \log_{10} (\mu_4 /M_\mathrm{Pl}) < 2$ & $-0.3$ & $-1.4$ \\
\noalign{\vskip 2pt}
%& & & & & \\
%Double well inflation & $\Lambda^4 \left( 1 - \frac{\phi^2}{\phi_0^2} \right)^2$ & $0.3 < \log_{10} (\phi_0 /M_\mathrm{Pl}) < 4.85$ & $2.6$ & $-3.8$ \\
%& & & & \\
D-brane inflation ($p=2$) & $\Lambda^4 \left( 1 - \mu^2_{{\rm D} \, 2} / \phi^p + \dots \right)$ & $- 6  < \log_{10} (\mu_{{\rm D} \, 2} /M_\mathrm{Pl}) < 0.3$ & $-2.3$ & $1.6$ \\
\noalign{\vskip 2pt}
%& & & & \\
D-brane inflation ($p=4$) & $\Lambda^4 \left( 1 - \mu^4_{{\rm D} \, 4} / \phi^p + \dots \right)$ & $- 6  < \log_{10} (\mu_{{\rm D} \, 4} /M_\mathrm{Pl}) < 0.3$ & $-2.2$ & $0.8$ \\
\noalign{\vskip 2pt}
%& & & & \\
Potential with exponential tails & $\Lambda^4 \left[ 1 - \exp{\left(-q \phi / M_\mathrm{Pl}\right)} + \dots \right]$ & $- 3  < \log_{10} q < 3$ & $-0.5$ & $-1.0$ \\
\noalign{\vskip 2pt}
%& & & & \\
Spontaneously broken SUSY & $\Lambda^4 \left[ 1 + \alpha_h \log \left(\phi / M_\mathrm{Pl}\right) + \dots  \right]$ & $- 2.5  < \log_{10} \alpha_h < 1$ & $9.0$ & $-5.0$ \\
\noalign{\vskip 2pt}
%& & & & \\
E-model $(n = 1)$ & $\Lambda^4 \left\{ 1 - \exp{\left[- \sqrt{2} \phi \left(\sqrt{3 \alpha_1^{\rm E}} M_\mathrm{Pl}\right)^{-1}\right] }\right\}^{2 n} $ & $-2 < \log_{10} \alpha_1^{\rm E} < 4$ & $0.2$ & $-1.0$ \\
\noalign{\vskip 2pt}
%& &  &  &  \\
E-model $(n = 2)$ & $\Lambda^4 \left\{ 1 - \exp{\left[- \sqrt{2} \phi \left(\sqrt{3 \alpha_2^{\rm E}} M_\mathrm{Pl}\right)^{-1}\right] }\right\}^{2 n} $ & $-2 < \log_{10} \alpha_2^{\rm E} < 4$ & $-0.1$ & $0.7$ \\
\noalign{\vskip 2pt}
%& &  &  &  \\
T-model $(m = 1)$ & $\Lambda^4 \tanh^{2 m} \left[ \phi \left(\sqrt{6 \alpha_1^{\rm T}} M_\mathrm{Pl}\right)^{-1}\right] $ & $-2 < \log_{10} \alpha_1^{\rm T} < 4$ & $-0.1$ & $0.1$ \\
\noalign{\vskip 2pt}
%& &  &  & \\
T-model $(m = 2)$ & $\Lambda^4 \tanh^{2 m} \left[ \phi \left(\sqrt{6 \alpha_2^{\rm T}} M_\mathrm{Pl}\right)^{-1}\right] $ & $-2 < \log_{10} \alpha_2^{\rm T} < 4$ & $-0.4$ & $0.1$ \\
%& &  &  &  \\
%& & & & \\
%Polynomial inflation & $\dots$ & $ \dots $ &     & \\
%                     &       & $ \dots $ & \dots & \dots \\
%& & & & \\
%Non-minimal coupling & & & \dots & \dots \\
\noalign{\vskip 2pt\hrule}
\end{tabular}
\end{center}
%\vspace{.4cm}
%\hspace{4cm}
\caption{\label{table:model_compar} 
Bayesian comparison for a selection of slow-roll inflationary models with $w_\mathrm{int}$ fixed (see text for more details). 
We quote 0.3 as the error on the Bayes factor. Models are strongly disfavoured when $\ln B < -5$. }
%{\bf Note that the extra column 
%with \Planck\ 2015 results will be removed when final results will be available since BAO will not be used for this analysis (only \Planck\ Legacy data).}}
\end{table*}
%\end{landscape}


==> Tables/table_inflationarymodels_v6.tex <==
%\newcommand{\pz}{\phantom{0}}
%\newcommand{\pzz}{\phantom{00}}
%\newcommand{\pd}{\phantom{-}}

%\begin{landscape}
\begin{table*}
\begin{center}
\footnotesize
%\scriptsize
%\begin{tabular}{lrrrrrrrr}
\begin{tabular}{lccc|c}
\hline
\vspace{.3cm}
%Inflationary & Potential & Prior(s) & $\Delta n$ & $\Delta\chi^2$& $\ln B$ \\
%Model & & & & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) \\  
Inflationary Model & Potential $V(\phi)$ & Prior(s) & $\Delta\chi^2$ & $\ln B$ \\
%& & & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) & ($w_\mathrm{int} = 0$) \\
& & & & \\
\noalign{\hrule\vskip 3pt}
%General models:
& & & & \\
$R + R^2/(6 M^2)$ & $\Lambda^4 \left( 1 - \exp{\left\{-\sqrt{2/3} \phi/M_\mathrm{pl}\right\}} \right)^2$ & None & ... & $ ... $ \\
& & & & \\
%\citep{Starobinsky:1980te,Mukhanov:1981xt,Starobinsky:1983zz}& & & & \\
%Power law potentials & $\Lambda^4 \left( \frac{\phi}{M_\mathrm{pl}} \right)^p$ & $0 \le p \le 4$ & ... & ... & $-$ \\
%\citep{Linde:1983gd} & & & & \\
%& & & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 2/3$ & $+5.0$ & $-4.6$ \\
& & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 1$ & $+6.9$ & $-3.9$ \\
& & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 4/3$ & $+13.3$ & $-6.2$ \\
& & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 2$ & $+26.0$ & $-11.8$ \\
& & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 3$ & $+52.5$ & $-13.3$ \\
& & & & \\
Power law potentials & $\Lambda^4 \left( \phi / M_\mathrm{pl} \right)^p$ & $p = 4$ & $-$ & $-56.1$ \\
& & & & \\
%\hline
Natural Inflation & $\Lambda^4 \left[ 1+\cos \left( \phi / f \right) \right]$ & $0.3 < \log_{10} \left(f/M_\mathrm{pl}\right) < 2.5$ & $+15.3$ & $-6.6$ \\
& & & & \\
Hilltop quadratic model ($p=2$) & $\Lambda^4 \left( 1 - \phi^2 / \mu_2^2 + ... \right)$ & $0.3 < \log_{10} (\mu_2 /M_\mathrm{pl}) < 4.85$ & $+0.0$ & $-$ \\
%\citep{Boubekeur:2005zm}
& & & & \\
Hilltop quartic model ($p=4$) & $\Lambda^4 \left( 1 - \phi^4 / \mu_4^4 + ... \right) $ & $-2 < \log_{10} (\mu_4 /M_\mathrm{pl}) < 2$ & $-0.7$ & $-$ \\
%& & & & & \\
%Double well inflation & $\Lambda^4 \left( 1 - \frac{\phi^2}{\phi_0^2} \right)^2$ & $0.3 < \log_{10} (\phi_0 /M_\mathrm{pl}) < 4.85$ & $2.6$ & $-3.8$ \\
& & & & \\
D-brane inflation ($p=2$) & $\Lambda^4 \left( 1 - \mu^2_{D \, 2} / \phi^2 + ... \right)$ & $- 6  < \log_{10} \left(\mu_{D \, 2} /M_\mathrm{pl}\right) < 0.3$ & $-4.0$ & $0.5$ \\
& & & & \\
D-brane inflation ($p=4$) & $\Lambda^4 \left( 1 - \mu^4_{D \, 4} / \phi^4 + ... \right)$ & $- 6  < \log_{10} \left(\mu_{D \, 4} /M_\mathrm{pl}\right) < 0.3$ & $-2.8$ & $-0.4$ \\
& & & & \\
Potential with exponential tails & $\Lambda^4 \left( 1 - \exp{\left\{-q \phi / M_\mathrm{pl}\right\}} + ... \right)$ & $- 3  < \log_{10} q < 0.3$ & $-0.8$ & $-1.0$ \\
& & & & \\
Spontaneously broken SUSY & $\Lambda^4 \left[ 1 + \alpha_h \log \left(\phi / M_\mathrm{pl}\right) + ...  \right]$ & $- 2.5  < \log_{10} \alpha_h < 1$ & $+5.6$ & $-6.8$ \\
& & & & \\
E-model $(n = 1)$ & $\Lambda^4 \left[ 1 - \exp{\left\{- \sqrt{2} \phi / \left(\sqrt{3 \alpha_1^E} M_\mathrm{pl}\right)\right\} }\right]^{2 n} $ & $0 < \log_{10} \alpha_1^E < 2$ & $-0.5$ & $-0.3$ \\
& &  &  &  \\
E-model $(n = 2)$ & $\Lambda^4 \left[ 1 - \exp{\left\{- \sqrt{2} \phi / \left(\sqrt{3 \alpha_2^E} M_\mathrm{pl}\right)\right\} }\right]^{2 n} $ & $0 < \log_{10} \alpha_2^E < 2$ & $-0.2$ & $-1.6$ \\
& &  &  &  \\
T-model $(m = 1)$ & $\Lambda^4 \tanh^{2 m} \left[ \phi / \left(\sqrt{6 \alpha_1^T} M_\mathrm{pl}\right) \right] $ & $0 < \log_{10} \alpha_1^T < 2$ & $-$ & $-1.2$ \\
& &  &  & \\
T-model $(m = 2)$ & $\Lambda^4 \tanh^{2 m} \left[ \phi / \left(\sqrt{6 \alpha_2^T} M_\mathrm{pl}\right) \right] $ & $0 < \log_{10} \alpha_2^T < 2$ & $-0.2$ & $-0.6$ \\
& &  &  &  \\
%& & & & \\
%Polynomial inflation & $...$ & $ ... $ &     & \\
%                     &       & $ ... $ & ... & ... \\
%& & & & \\
%Non-minimal coupling & & & ... & ... \\
\noalign{\vskip 2pt\hrule}
\end{tabular}
\end{center}
%\vspace{.4cm}
%\hspace{4cm}
\caption{\label{table:model_compar} 
Bayesian comparison for a selection of slow-roll inflationary models with $w_\mathrm{int}$ fixed (see text for more details). 
We quote 0.3 as error on the Bayes factor.}
\end{table*}
%\end{landscape}

